Wisdom of the Crowds or Ignorance of the Masses? A data-driven guide to WSB

A trite yet fundamental question in economics is: What causes large asset price fluctuations? A tenfold rise in the price of GameStop equity, between the 22nd and 28th of January 2021, demonstrated that herding behaviour among retail investors is an important contributing factor. This paper presents a data-driven guide to the forum that started the hype -- WallStreetBets (WSB). Our initial experiments decompose the forum using a large language topic model and network tools. The topic model describes the evolution of the forum over time and shows the persistence of certain topics (such as the market / S\&P500 discussion), and the sporadic interest in others, such as COVID or crude oil. Network analysis allows us to decompose the landscape of retail investors into clusters based on their posting and discussion habits; several large, correlated asset discussion clusters emerge, surrounded by smaller, niche ones. A second set of experiments assesses the impact that WSB discussions have had on the market. We show that forum activity has a Granger-causal relationship with the returns of several assets, some of which are now commonly classified as `meme stocks', while others have gone under the radar. The paper extracts a set of short-term trade signals from posts and long-term (monthly and weekly) trade signals from forum dynamics, and considers their predictive power at different time horizons. In addition to the analysis, the paper presents the dataset, as well as an interactive dashboard, in order to promote further research.

==> Sections/5.1Results_hype.tex <==
\section{What drives popularity on WSB?}
\label{sec:results_popularity}

\paragraph{Heavy-tailed nature of attention on WSB}

\paragraph{Returns predictive of popularity}



==> Sections/5.3Results_topic_modelling.tex <==
\subsection{WSB discussions and markets}
\label{sec:results_returns}


% what is the language associated with popularity ? --> scalat to N detection 

\paragraph{Initial exploration}

%\input{Tables/return_stats}
In this analysis, we look at the results of the topic model presented in the Data section.
%add ref to the data section 

There is a wide literature discussing the strong links between market volatility and uncertainty of the informational ecosystem. Changes in topic mentions and sentiments associated with economic news are associated with heightened market volatility \cite{Nyman2018NewsAN}. Agreement between multiple large-scale news outlets also seems to form a good correlate for market uncertainty as measured by market volatility \cite{pivskorec2014cohesiveness}. The central intuition is that agents collect information from a given range of sources and these sources cover various sources of risk. When agents diversify their risk collection, they are less likely to react rashly to adverse market movements. A reduction in the span of risks covered, as newspapers all simultaneous talk about the same breaking news topic such as a global pandemic or war for instance,  can leave the market in a heightened state of vulnerability as the ability of its agents to collect diverse information has deteriorated. 

We chose to test out this hypothesis by building a metric to capture the range of topics being discussed on the forum. We begin from the topic distribution, displayed in Figure \ref{fig:top_30_topics_overtime}, which considers the fraction of attention paid to a given topic on the forum over time. The metric we choose to calculate the degree to which the landscape is dominated by one single topic is Shannon entropy. Shannon entropy gives us, for each month, how surprised should we be to get a topic by sampling randomly across all the posts of that month.  Since each topic is taken as covering a distinct representative slice of the overall discourse on the platform, one dominating topic could imply that the entire forum's activity would be devoted to little else and the information-gathering ability of its' members might be affected as a result. 

Conversely, the observations in prior sections have also led us to suspect that the WSB forum reacts to current market movements rather than forewarns it. 

We therefore chose to test to what extent the entropy can be used to forecast next time-period volatility.  

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{Figures/Shannon_entropy.png}
%    \caption{\textbf{Topic Shannon Entropy overtime}}
%    \label{fig:entropy}
%\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/VIX_vs_entropy.png}
    \caption{\textbf{Topic Shannon Entropy over time and the VIX index correlate}}

    \label{fig:vix-entropy}
\end{figure}

The entropy metric presented blue in \ref{fig:vix-entropy} represents the often sharp fluctuations of the diversity of topics represented in WSB. It is shown to correlate strongly with the CBOE VIX index, a metric of market uncertainty.

However, when run in a regression setting trying to explain the next month VIX, it fails to explain future period VIX. 

We can interpret this failure to provide an explanation for out of sample volatility in two ways : 1. The forum is broadly reactive to market movements as evidenced previously in the CAR plots. Because, we did not have enough data to run this topic model with any granularity lower than the month we cannot discount the possibility that the market may have moved during the month and the topic coverage shifted to reflect that rather than the other way around. 2. The topic  the WSB and news media ecosystem are different and wsb does not capture the entirety of the information gathering being done.

\begin{center}
\begin{tabular}{lclc}
\toprule
\textbf{Dep. Variable:}    &   shifted\_vol   & \textbf{  R-squared:         } &     0.493   \\
\textbf{Model:}            &       OLS        & \textbf{  Adj. R-squared:    } &     0.480   \\
\textbf{Method:}           &  Least Squares   & \textbf{  F-statistic:       } &     36.04   \\
\textbf{Date:}             & Wed, 26 Apr 2023 & \textbf{  Prob (F-statistic):} &  1.18e-11   \\
\textbf{Time:}             &     00:40:43     & \textbf{  Log-Likelihood:    } &   -240.25   \\
\textbf{No. Observations:} &          77      & \textbf{  AIC:               } &     486.5   \\
\textbf{Df Residuals:}     &          74      & \textbf{  BIC:               } &     493.5   \\
\textbf{Df Model:}         &           2      & \textbf{                     } &             \\
\textbf{Covariance Type:}  &    nonrobust     & \textbf{                     } &             \\
\bottomrule
\end{tabular}
\begin{tabular}{lcccccc}
                   & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P$> |$t$|$} & \textbf{[0.025} & \textbf{0.975]}  \\
\midrule
\textbf{const}     &      12.1893  &        6.429     &     1.896  &         0.062        &       -0.620    &       24.999     \\
\textbf{Adj Close} &       0.6656  &        0.088     &     7.579  &         0.000        &        0.491    &        0.841     \\
\textbf{entropy}   &      -2.4950  &        2.328     &    -1.072  &         0.287        &       -7.133    &        2.143     \\
\bottomrule
\end{tabular}
\begin{tabular}{lclc}
\textbf{Omnibus:}       & 29.382 & \textbf{  Durbin-Watson:     } &    1.869  \\
\textbf{Prob(Omnibus):} &  0.000 & \textbf{  Jarque-Bera (JB):  } &   78.686  \\
\textbf{Skew:}          &  1.198 & \textbf{  Prob(JB):          } & 8.19e-18  \\
\textbf{Kurtosis:}      &  7.334 & \textbf{  Cond. No.          } &     211.  \\
\bottomrule
\end{tabular}
%\caption{OLS Regression Results}
\end{center}

Notes: \newline
 [1] Standard Errors assume that the covariance matrix of the errors is correctly specified.

%\paragraph{Investor Clusters} 
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{Figures/submission_similarity.pdf}
%    \caption{\textbf{Ticker Discussion Clusters:} We create a weighted network between tickers where an edge exists from ticker A to ticker B if at least twenty percent of authors who create submissions about ticker B also post about ticker A. Clusters are extracted using the Leiden algorithm \citep{traag2019louvain}. }
%    \label{fig:my_label}
%\end{figure}

%        \begin{figure}[ht]
%                \begin{subfigure}{.51\textwidth}
%                \centering
%                \frame{\includegraphics[width=\linewidth]{Figures/investor_clusters.pdf}}
%                \caption{Investor clusters on WSB} 
%                \label{fig:investor_clusters}
%            \end{subfigure}
%            \hfill
%            \begin{subfigure}{.48\textwidth}
%                \centering
%                \frame{\includegraphics[width=\linewidth]{Figures/distributions.pdf}}
%                \caption{A sample screenshot of user profits} 
%                \label{fig:cluster_returns}
%            \end{subfigure}
%            \caption{\textbf{Clusters on WSB}}
%            \label{fig:clusters_and_profits}
%        \end{figure} 
    




==> Tables/dd_fe_results.tex <==
\begin{tabular}{llllll}
\toprule
 &  &  &  & Net DD & Previous day return \\
Sample & Obs & Flaired & Lookahead &  &  \\
\midrule
All data & 685438 & True & Four weeks & -0.012 & -0.056 \\
% \cline{1-6} \cline{2-6} \cline{3-6}
 &  &  &  & $(0.0076)$ & $(0.0197)^{**}$ \\
 &  &  & Twelve weeks & 0.011 & -0.080 \\
 &  &  &  & $(0.0274)$ & $(0.0288)^{**}$ \\
 &  &  & 26 weeks & 0.016 & -0.068 \\
 &  &  &  & $(0.0363)$ & $(0.0358)$ \\
\cline{3-6}
 &  & False & Four weeks & -0.009 & -0.056 \\
% \cline{3-6}
 &  &  &  & $(0.0066)$ & $(0.0197)^{**}$ \\
 &  &  & Twelve weeks & 0.017 & -0.080 \\
 &  &  &  & $(0.0283)$ & $(0.0288)^{**}$ \\
 &  &  & 26 weeks & 0.021 & -0.068 \\
 &  &  &  & $(0.0346)$ & $(0.0358)$ \\
\cline{1-6}
Pre-2021, all stocks & 561414 & True & Four weeks & -0.001 & -0.059 \\
% \cline{1-6} \cline{2-6} \cline{3-6}
 &  &  &  & $(0.0061)$ & $(0.0197)^{**}$ \\
 &  &  & Twelve weeks & 0.001 & -0.077 \\
 &  &  &  & $(0.0118)$ & $(0.0299)^{**}$ \\
 &  &  & 26 weeks & 0.003 & -0.066 \\
 &  &  &  & $(0.0226)$ & $(0.0366)$ \\
\cline{3-6}
 &  & False & Four weeks & 0.007 & -0.059 \\
% \cline{3-6}
 &  &  &  & $(0.0065)$ & $(0.0197)^{**}$ \\
 &  &  & Twelve weeks & 0.011 & -0.077 \\
 &  &  &  & $(0.0151)$ & $(0.0299)^{**}$ \\
 &  &  & 26 weeks & 0.012 & -0.066 \\
 &  &  &  & $(0.0259)$ & $(0.0365)$ \\
\cline{1-6} 
Pre-2021, no meme & 558888 & True & Four weeks & -0.000 & -0.059 \\
% \cline{1-6} \cline{2-6} \cline{3-6}
 &  &  &  & $(0.0057)$ & $(0.0198)^{**}$ \\
 &  &  & Twelve weeks & -0.007 & -0.076 \\
 &  &  &  & $(0.0096)$ & $(0.0299)^{*}$ \\
 &  &  & 26 weeks & -0.015 & -0.067 \\
 &  &  &  & $(0.0153)$ & $(0.0363)$ \\
\cline{3-6}
 &  & False & Four weeks & 0.004 & -0.059 \\
% \cline{3-6}
 &  &  &  & $(0.0054)$ & $(0.0198)^{**}$ \\
 &  &  & Twelve weeks & -0.003 & -0.076 \\
 &  &  &  & $(0.0089)$ & $(0.0299)^{*}$ \\
 &  &  & 26 weeks & -0.012 & -0.067 \\
 &  &  &  & $(0.0144)$ & $(0.0363)$ \\
\cline{1-6} 
2021, all stocks & 124024 & True & Four weeks & -0.050 & -0.039 \\
% \cline{1-6} \cline{2-6} \cline{3-6}
 &  &  &  & $(0.0217)^{*}$ & $(0.0613)$ \\
 &  &  & Twelve weeks & 0.045 & -0.094 \\
 &  &  &  & $(0.0802)$ & $(0.0855)$ \\
 &  &  & 26 weeks & 0.058 & -0.080 \\
 &  &  &  & $(0.0781)$ & $(0.1121)$ \\
\cline{3-6}
 &  & False & Four weeks & -0.041 & -0.038 \\
% \cline{3-6}
 &  &  &  & $(0.0137)^{**}$ & $(0.061)$ \\
 &  &  & Twelve weeks & 0.030 & -0.094 \\
 &  &  &  & $(0.0555)$ & $(0.0855)$ \\
 &  &  & 26 weeks & 0.039 & -0.080 \\
 &  &  &  & $(0.0517)$ & $(0.1121)$ \\
\cline{1-6}
2021, no meme & 123478 & True & Four weeks & -0.054 & -0.028 \\
% \cline{1-6} \cline{2-6} \cline{3-6}
 &  &  &  & $(0.0165)^{**}$ & $(0.0601)$ \\
 &  &  & Twelve weeks & -0.091 & -0.093 \\
 &  &  &  & $(0.0218)^{***}$ & $(0.0879)$ \\
 &  &  & 26 weeks & -0.105 & -0.086 \\
 &  &  &  & $(0.0329)^{**}$ & $(0.117)$ \\
\cline{3-6}
 &  & False & Four weeks & -0.039 & -0.028 \\
% \cline{3-6}
 &  &  &  & $(0.0105)^{***}$ & $(0.0601)$ \\
 &  &  & Twelve weeks & -0.070 & -0.093 \\
 &  &  &  & $(0.017)^{***}$ & $(0.0879)$ \\
 &  &  & 26 weeks & -0.080 & -0.085 \\
 &  &  &  & $(0.0252)^{**}$ & $(0.117)$ \\
% \cline{1-6} \cline{2-6} \cline{3-6}
\bottomrule
\end{tabular}



==> bibliography_dragos.tex <==
@article{tucker2018social,
  title={Social media, political polarization, and political disinformation: A review of the scientific literature},
  author={Tucker, Joshua A and Guess, Andrew and Barber{\'a}, Pablo and Vaccari, Cristian and Siegel, Alexandra and Sanovich, Sergey and Stukal, Denis and Nyhan, Brendan},
  journal={Political polarization, and political disinformation: a review of the scientific literature (March 19, 2018)},
  year={2018}
}

@article{vosoughi2018spread,
  title={The spread of true and false news online},
  author={Vosoughi, Soroush and Roy, Deb and Aral, Sinan},
  journal={Science},
  volume={359},
  number={6380},
  pages={1146--1151},
  year={2018},
  publisher={American Association for the Advancement of Science}
}

@book{lehmann2018complex,
  title={Complex spreading phenomena in social systems},
  author={Lehmann, Sune and Ahn, Yong-Yeol},
  year={2018},
  publisher={Springer}
}

@article{black1986noise,
  title={Noise},
  author={Black, Fischer},
  journal={The journal of finance},
  volume={41},
  number={3},
  pages={528--543},
  year={1986},
  publisher={Wiley Online Library}
}

@article{semenova2021reddit,
  title={Reddit's self-organised bull runs: Social contagion and asset prices},
  author={Semenova, Valentina and Winkler, Julian},
  journal={arXiv preprint arXiv:2104.01847},
  year={2021}
}

@article{shleifer1990noise,
  title={The noise trader approach to finance},
  author={Shleifer, Andrei and Summers, Lawrence H},
  journal={Journal of Economic perspectives},
  volume={4},
  number={2},
  pages={19--33},
  year={1990}
}

@article{shefrin1994behavioral,
  title={Behavioral capital asset pricing theory},
  author={Shefrin, Hersh and Statman, Meir},
  journal={Journal of financial and quantitative analysis},
  volume={29},
  number={3},
  pages={323--349},
  year={1994},
  publisher={Cambridge University Press}
}

@article{de1990noise,
  title={Noise trader risk in financial markets},
  author={De Long, J Bradford and Shleifer, Andrei and Summers, Lawrence H and Waldmann, Robert J},
  journal={Journal of political Economy},
  volume={98},
  number={4},
  pages={703--738},
  year={1990},
  publisher={The University of Chicago Press}
}

@article{hommes2021behavioral,
    Author = {Hommes, Cars},
    Title = {Behavioral and Experimental Macroeconomics and Policy Analysis: A Complex Systems Approach},
    Journal = {Journal of Economic Literature},
    Volume = {59},
    Number = {1},
    Year = {2021},
    Month = {March},
    Pages = {149-219},
}

@article{bradley21wsb,
   author = {Bradley, Daniel and Hanousek Jr, Jan and Jame, Russell and Xiao, Zicheng},
   title = {Place Your Bets? The Market Consequences of Investment Advice on Reddit's Wallstreetbets},
   journal = {The Market Consequences of Investment Advice on Reddit's Wallstreetbets (March 15, 2021)},
   year = {2021},
   type = {Journal Article}
}

@article{Buz2021wsb,
   author = {Buz, Tolga and de Melo, Gerard},
   title = {Should You Take Investment Advice From WallStreetBets? A Data-Driven Approach},
   journal = {arXiv preprint arXiv:2105.02728},
   year = {2021},
   type = {Journal Article}
}


@article{bollen2011twitter,
    title = "Twitter mood predicts the stock market",
    journal = "Journal of Computational Science",
    volume = "2",
    number = "1",
    pages = "1 - 8",
    year = "2011",
    author = "Johan Bollen and Huina Mao and Xiaojun Zeng",
}

@article{gentzkow2019text,
    Author = {Gentzkow, Matthew and Kelly, Bryan and Taddy, Matt},
    Title = {Text as Data},
    Journal = {Journal of Economic Literature},
    Volume = {57},
    Number = {3},
    Year = {2019},
    Month = {September},
    Pages = {535-74}
}

@article{Duz2021,
author = {Selin Duz Tan and Oktay Tas},
title = {Social Media Sentiment in International Stock Returns and Trading Activity},
journal = {Journal of Behavioral Finance},
volume = {22},
number = {2},
pages = {221-234},
year  = {2021},
publisher = {Routledge},
doi = {10.1080/15427560.2020.1772261},

URL = { 
        https://doi.org/10.1080/15427560.2020.1772261
    
},
eprint = { 
        https://doi.org/10.1080/15427560.2020.1772261
    
}

}



@article{traag2019louvain,
  title={From Louvain to Leiden: guaranteeing well-connected communities},
  author={Traag, Vincent A and Waltman, Ludo and Van Eck, Nees Jan},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={5233},
  year={2019},
  publisher={Nature Publishing Group UK London}
}


@article{Wan2021,
   author = {Wan, Xingchen and Yang, Jie and Marinov, Slavi and Calliess, Jan-Peter and Zohren, Stefan and Dong, Xiaowen},
   title = {Sentiment correlation in financial news networks and associated market movements},
   journal = {Scientific Reports},
   volume = {11},
   number = {1},
   pages = {3062},
   abstract = {In an increasingly connected global market, news sentiment towards one company may not only indicate its own market performance, but can also be associated with a broader movement on the sentiment and performance of other companies from the same or even different sectors. In this paper, we apply NLP techniques to understand news sentiment of 87 companies among the most reported on Reuters for a period of 7 years. We investigate the propagation of such sentiment in company networks and evaluate the associated market movements in terms of stock price and volatility. Our results suggest that, in certain sectors, strong media sentiment towards one company may indicate a significant change in media sentiment towards related companies measured as neighbours in a financial network constructed from news co-occurrence. Furthermore, there exists a weak but statistically significant association between strong media sentiment and abnormal market return as well as volatility. Such an association is more significant at the level of individual companies, but nevertheless remains visible at the level of sectors or groups of companies.},
   ISSN = {2045-2322},
   DOI = {10.1038/s41598-021-82338-6},
   url = {https://doi.org/10.1038/s41598-021-82338-6},
   year = {2021},
   type = {Journal Article}
}

@article{araci2019finbert,
  title={Finbert: Financial sentiment analysis with pre-trained language models},
  author={Araci, Dogu},
  journal={arXiv preprint arXiv:1908.10063},
  year={2019}
}

@article{zhang19,
   author = {Zhang, Zihao and Zohren, Stefan and Roberts, Stephen},
   title = {DeepLOB: Deep Convolutional Neural Networks for Limit Order Books},
   journal = {IEEE Transactions on Signal Processing},
   volume = {67},
   number = {11},
   pages = {3001-3012},
   DOI = {10.1109/TSP.2019.2907260},
   year = {2019},
   type = {Journal Article}
}

% social media and markets articles
% positive
@article{Chen14Wisdom,
    author = {Chen, Hailiang and De, Prabuddha and Hu, Yu (Jeffrey) and Hwang, Byoung-Hyoun},
    title = "{Wisdom of Crowds: The Value of Stock Opinions Transmitted Through Social Media}",
    journal = {The Review of Financial Studies},
    volume = {27},
    number = {5},
    pages = {1367-1403},
    year = {2014},
    month = {02},
    abstract = "{Social media has become a popular venue for individuals to share the results of their own analysis on financial securities. This paper investigates the extent to which investor opinions transmitted through social media predict future stock returns and earnings surprises. We conduct textual analysis of articles published on one of the most popular social media platforms for investors in the United States. We also consider the readers' perspective as inferred via commentaries written in response to these articles. We find that the views expressed in both articles and commentaries predict future stock returns and earnings surprises.}",
    issn = {0893-9454},
    doi = {10.1093/rfs/hhu001},
    url = {https://doi.org/10.1093/rfs/hhu001},
    eprint = {https://academic.oup.com/rfs/article-pdf/27/5/1367/24449504/hhu001.pdf},
}

@INPROCEEDINGS{PagoluTwitterSent,

  author={Pagolu, Venkata Sasank and Reddy, Kamal Nayan and Panda, Ganapati and Majhi, Babita},

  booktitle={2016 International Conference on Signal Processing, Communication, Power and Embedded System (SCOPES)}, 

  title={Sentiment analysis of Twitter data for predicting stock market movements}, 

  year={2016},

  volume={},

  number={},

  pages={1345-1350},

  doi={10.1109/SCOPES.2016.7955659}}


@article{FARRELL2022616,
title = {The democratization of investment research and the informativeness of retail investor trading},
journal = {Journal of Financial Economics},
volume = {145},
number = {2, Part B},
pages = {616-641},
year = {2022},
issn = {0304-405X},
doi = {https://doi.org/10.1016/j.jfineco.2021.07.018},
url = {https://www.sciencedirect.com/science/article/pii/S0304405X21004050},
author = {Michael Farrell and T. Clifton Green and Russell Jame and Stanimir Markov},
keywords = {Investment research, Seeking alpha, Retail investors, Informed trading},
abstract = {We study the effects of social media on the informativeness of retail trading. Our identification strategy exploits the editorial delay between report submission and publication on Seeking Alpha, a popular crowdsourced investment research platform. We find the ability of retail order imbalances to predict the cross-section of stock returns and cash-flow news increases sharply in the intraday post-publication window relative to the pre-publication window. The findings are robust to controlling for report tone and stronger for reports authored by more capable contributors. The evidence suggests that recent technology-enabled innovations in how individuals share information help retail investors become better informed.}
}

@article{TwitterSentiment1,
  title={Analyzing stock market movements using twitter sentiment analysis},
  author={Rao, Tushar and Srivastava, Saket and others},
  year={2012},
  publisher={IEEE Computer Society}
}

@article{TwitterSentiment2,
author = {Sul, Hong Kee and Dennis, Alan R. and Yuan, Lingyao (Ivy)},
title = {Trading on Twitter: Using Social Media Sentiment to Predict Stock Returns},
journal = {Decision Sciences},
volume = {48},
number = {3},
pages = {454-488},
keywords = {Twitter, Emotion, Sentiment, Stock returns, S&P500},
doi = {https://doi.org/10.1111/deci.12229},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/deci.12229},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/deci.12229},
abstract = {ABSTRACT Decision making is often based on the rational assessment of information, but recent research shows that emotional sentiment also plays an important role, especially for investment decision making. Emotional sentiment about a firm's stock that spreads rapidly through social media is more likely to be incorporated quickly into stock prices (e.g., on the same trading day it was expressed), while sentiment that spreads slowly takes longer to be incorporated into stock prices and thus is more likely to predict stock prices on future days. We analyzed the cumulative sentiment (positive and negative) in 2.5 million Twitter postings about individual S\&P 500 firms and compared this to the stock returns of those firms. Our results show that the sentiment in tweets about a specific firm from users with less than 171 followers (the median in our sample) had a significant impact on the stock's returns on the next trading day, the next 10 days, and the next 20 days. Interestingly, sentiment in tweets from users with fewer than 171 followers that were not retweeted had the greatest impact on future stock returns. A trading strategy based on these findings produced meaningful economic gains on the order of an 11–15\% annual return.},
year = {2017}
}

% Negative
@article{cookson2022echo,
  title={Echo chambers},
  author={Cookson, J Anthony and Engelberg, Joseph and Mullins, William},
  journal={Available at SSRN 3603107},
  year={2022},
  abstract={We find evidence of selective exposure to confirmatory information among 400,000 users on
the investor social network StockTwits. Self-described bulls are 5 times more likely to follow a
user with a bullish view of the same stock than self-described bears. Consequently, bulls see 62
more bullish messages and 24 fewer bearish messages than bears over the same 50-day period.
These “echo chambers” exist even among professional investors and are strongest for investors
who trade on their beliefs. Finally, beliefs formed in echo chambers are associated with lower
ex-post returns, more siloing of information and more trading volume.}
}

@article{mergerrumors,
title = {Can social media distort price discovery? Evidence from merger rumors},
journal = {Journal of Accounting and Economics},
volume = {70},
number = {1},
pages = {101334},
year = {2020},
issn = {0165-4101},
doi = {https://doi.org/10.1016/j.jacceco.2020.101334},
url = {https://www.sciencedirect.com/science/article/pii/S0165410120300367},
author = {Weishi Jia and Giulia Redigolo and Susan Shu and Jingran Zhao},
keywords = {Social media, Twitter, Merger and acquisition, Rumor, Merger rumor, Persuasion bias},
abstract = {We study whether social media can play a negative information role by impeding price discovery in the presence of highly speculative rumors. We focus on merger rumors, where most do not materialize. We find that merger rumors accompanied by greater Twitter activity elicit greater immediate market reaction even though rumor-related Twitter activity is unrelated to the probability of merger realization. The price distortion associated with tweet volume persists weeks after a rumor and reverses only after eight weeks. The price distortion is more pronounced for rumors tweeted by Twitter users with greater social influence, for target firms with low institutional ownership, and for rumors that supply more details. Our evidence suggests that social media can be a rumor mill that hinders the market's price discovery of potentially false information.}
}

@article{KIM2014708,
title = {Investor sentiment from internet message postings and the predictability of stock returns},
journal = {Journal of Economic Behavior & Organization},
volume = {107},
pages = {708-729},
year = {2014},
note = {Empirical Behavioral Finance},
issn = {0167-2681},
doi = {https://doi.org/10.1016/j.jebo.2014.04.015},
url = {https://www.sciencedirect.com/science/article/pii/S0167268114001206},
author = {Soon-Ho Kim and Dongcheol Kim},
keywords = {Investor sentiment, Return predictability, Internet posting messages, Text classification, Volatility, Trading volume},
abstract = {By using an extensive dataset of more than 32 million messages on 91 firms posted on the Yahoo! Finance message board over the period January 2005 to December 2010, we examine whether investor sentiment as expressed in posted messages has predictive power for stock returns, volatility, and trading volume. In intertemporal and cross-sectional regression analyses, we find no evidence that investor sentiment forecasts future stock returns either at the aggregate or at the individual firm level. Rather, we find evidence that investor sentiment is positively affected by prior stock price performance. We also find no significant evidence that investor sentiment from Internet postings has predictive power for volatility and trading volume. A distinctive feature of our study is the use of sentiment information explicitly revealed by retail investors as well as classified by a machine learning classification algorithm and a much longer sample period relative to prior studies.}
}

% negative end

% mixed

@article{GIANNINI201994,
title = {The convergence and divergence of investors' opinions around earnings news: Evidence from a social network},
journal = {Journal of Financial Markets},
volume = {42},
pages = {94-120},
year = {2019},
issn = {1386-4181},
doi = {https://doi.org/10.1016/j.finmar.2018.12.003},
url = {https://www.sciencedirect.com/science/article/pii/S1386418117300095},
author = {Robert Giannini and Paul Irvine and Tao Shu},
keywords = {Investor disagreement, Social media, Divergence of opinion, Convergence of opinion, Trading volume, Stock returns, Earnings announcement},
abstract = {We collect a unique dataset of Twitter posts to examine the change in investor disagreement around earnings announcements. We find that investors' opinions can either converge (reduced disagreement) or diverge (increased disagreement) around earnings announcements. The convergence and divergence of opinion has significant effects on trading volume and return. Consistent with theoretical predictions, both the convergence and divergence of opinion are associated with a greater volume reaction to earnings news. While the convergence of opinion is associated with lower earnings announcement returns, the divergence of opinion is associated with higher earnings announcement returns.}
}
%
@inproceedings{node2vec,
author = {Grover, Aditya and Leskovec, Jure},
title = {Node2vec: Scalable Feature Learning for Networks},
year = {2016},
isbn = {9781450342322},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2939672.2939754},
doi = {10.1145/2939672.2939754},
abstract = {Prediction tasks over nodes and edges in networks require careful effort in engineering features used by learning algorithms. Recent research in the broader field of representation learning has led to significant progress in automating prediction by learning the features themselves. However, present feature learning approaches are not expressive enough to capture the diversity of connectivity patterns observed in networks. Here we propose node2vec, an algorithmic framework for learning continuous feature representations for nodes in networks. In node2vec, we learn a mapping of nodes to a low-dimensional space of features that maximizes the likelihood of preserving network neighborhoods of nodes. We define a flexible notion of a node's network neighborhood and design a biased random walk procedure, which efficiently explores diverse neighborhoods. Our algorithm generalizes prior work which is based on rigid notions of network neighborhoods, and we argue that the added flexibility in exploring neighborhoods is the key to learning richer representations.We demonstrate the efficacy of node2vec over existing state-of-the-art techniques on multi-label classification and link prediction in several real-world networks from diverse domains. Taken together, our work represents a new way for efficiently learning state-of-the-art task-independent representations in complex networks.},
booktitle = {Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {855–864},
numpages = {10},
keywords = {information networks, node embeddings, feature learning, graph representations},
location = {San Francisco, California, USA},
series = {KDD '16}
}

 @misc{ponciano_2021, title={Meme Stock Saga officially over? gamestop short interest plunged 70\% amid \$20 billion loss}, url={https://www.forbes.com/sites/jonathanponciano/2021/02/10/meme-stock-saga-officially-over-gamestop-short-interest-plunged-70-amid-20-billion-loss/?sh=138c22eb2130}, journal={Forbes}, publisher={Forbes Magazine}, author={Ponciano, Jonathan}, year={2021}, month={Feb}} 
 


@article{noise,
author = {De Long, J. Bradford and Shleifer, Andrei and Summers, Lawrence H. and Waldmann, Robert J.},
title = {Noise Trader Risk in Financial Markets},
journal = {Journal of Political Economy},
volume = {98},
number = {4},
pages = {703-738},
year = {1990},
doi = {10.1086/261703},

URL = { 
        https://doi.org/10.1086/261703
    
},
eprint = { 
        https://doi.org/10.1086/261703
    
}
,
    abstract = { We present a simple overlapping generations model of an asset market in which irrational noise traders with erroneous stochastic beliefs both affect prices and earn higher expected returns. The unpredictability of noise traders' beliefs creates a risk in the price of the asset that deters rational arbitrageurs from aggressively betting against them. As a result, prices can diverge significantly from fundamental values even in the absence of fundamental risk. Moreover, bearing a disproportionate amount of risk that they themselves create enables noise traders to earn a higher expected return than rational investors do. The model sheds light on a number of financial anomalies, including the excess volatility of asset prices, the mean reversion of stock returns, the underpricing of closed-end mutual funds, and the Mehra-Prescott equity premium puzzle. }
}

@article{black,
author = {BLACK, FISCHER},
title = {Noise},
journal = {The Journal of Finance},
volume = {41},
number = {3},
pages = {528-543},
doi = {https://doi.org/10.1111/j.1540-6261.1986.tb04513.x},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/j.1540-6261.1986.tb04513.x},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1540-6261.1986.tb04513.x},
abstract = {ABSTRACT The effects of noise on the world, and on our views of the world, are profound. Noise in the sense of a large number of small events is often a causal factor much more powerful than a small number of large events can be. Noise makes trading in financial markets possible, and thus allows us to observe prices for financial assets. Noise causes markets to be somewhat inefficient, but often prevents us from taking advantage of inefficiencies. Noise in the form of uncertainty about future tastes and technology by sector causes business cycles, and makes them highly resistant to improvement through government intervention. Noise in the form of expectations that need not follow rational rules causes inflation to be what it is, at least in the absence of a gold standard or fixed exchange rates. Noise in the form of uncertainty about what relative prices would be with other exchange rates makes us think incorrectly that changes in exchange rates or inflation rates cause changes in trade or investment flows or economic activity. Most generally, noise makes it very difficult to test either practical or academic theories about the way that financial or economic markets work. We are forced to act largely in the dark.},
year = {1986}
}

@article{Fama,
 ISSN = {00221082, 15406261},
 URL = {http://www.jstor.org/stable/2325486},
 author = {Eugene F. Fama},
 journal = {The Journal of Finance},
 number = {2},
 pages = {383--417},
 publisher = {[American Finance Association, Wiley]},
 title = {Efficient Capital Markets: A Review of Theory and Empirical Work},
 urldate = {2022-09-05},
 volume = {25},
 year = {1970}
}



 @misc{armstrong_2021, title={R/wallstreetbets throws down challenge to regulators}, url={https://www.ft.com/content/8a483767-6b55-40a2-b8a6-1439a2f56084}, journal={Subscribe to read | Financial Times}, publisher={Financial Times}, author={Armstrong, Robert}, year={2021}, month={Jan}} 

@article{COSTOLA2021110021,
title = {On the “mementum” of meme stocks},
journal = {Economics Letters},
volume = {207},
pages = {110021},
year = {2021},
issn = {0165-1765},
doi = {https://doi.org/10.1016/j.econlet.2021.110021},
url = {https://www.sciencedirect.com/science/article/pii/S0165176521002986},
author = {Michele Costola and Matteo Iacopini and Carlo R.M.A. Santagiustina},
keywords = {Meme stocks, Social media, Social trading, Cointegration, Regime switching},
abstract = {The meme stock phenomenon has yet to be explored. In this note, we provide evidence that these stocks display common stylized facts for the dynamics of price, trading volume, and social media activity. Using a regime-switching cointegration model, we identify the meme stock “mementum” which exhibits a different characterization compared to other stocks with high volumes of activity (persistent and not) on social media. Finally, we show that mementum is significant and positively related to the stock’s returns. Understanding these properties helps investors and market authorities in their decisions.}
}

@inproceedings{gao2021review,
  title={A review of natural language processing for financial technology},
  author={Gao, Ruizhuo and Zhang, Zeqi and Shi, Zhenning and Xu, Dan and Zhang, Weijuan and Zhu, Dewei},
  booktitle={International Symposium on Artificial Intelligence and Robotics 2021},
  volume={11884},
  pages={262--277},
  year={2021},
  organization={SPIE}
}

%WSB literature

@article{boylston2021wallstreetbets,
  title={Wallstreetbets: positions or ban},
  author={Boylston, Christian and Palacios, Beatriz and Tassev, Plamen and Bruckman, Amy},
  journal={arXiv preprint arXiv:2101.12110},
  abstract={r/wallstreetbets (WallStreetBets or WSB) is a subreddit devoted to irreverent memes and high-risk options trading. As of March 30, 2020, the subreddit boasts a usership of nearly 1.1 millions subscribers and self-describes as "if 4chan found a Bloomberg terminal." This paper will utilize Amy Jo Kim's community design principles along with social psychology theory as frameworks to understand how this chaotic, oftentimes offensive community has developed one of the largest and most loyal user bases on the platform. We will further argue that humor plays a vital role in promoting in-group cohesion and in providing an unconventional third place for traders (and thinly veiled gamblers) to seek support from each other in the form of vulgar, yet good-humored taunting.},
  year={2021}
}

 @article{reijmer2021contagion,
  title={Contagion of Narratives: An Example of the WallStreetBets Saga},
  author={Reijmer, Niek},
  year={2021}
}

@inproceedings{wang2021predicting,
  title = {Predicting \$ gme stock price movement using sentiment from reddit r/wallstreetbets},
  author={Wang, Charlie and Luo, Ben},
  booktitle={Proceedings of the Third Workshop on Financial Technology and Natural Language Processing},
  pages={22--30},
  year={2021},
  abstract={In early 2021, GameStop’s (NYSE: GME) stock underwent a prolonged period of rapid, drastic fluctuations in price resulting from a short squeeze orchestrated by the r/wallstreetbets community on Reddit. In this paper, we present our experiments and findings for predicting the direction of GME’s daily price movement using sentiment from r/wallstreetbets posts. We use VADER for automatic sentiment analysis combined with word2vec and BERT semantic representations, and experiment with a variety of classifier models, including both
traditional ML and deep learning approaches.},
}

@article{anand2021wallstreetbets,
  title={WallStreetBets against wall street: The Role of reddit in the GameStop short squeeze},
  author={Anand, Abhinav and Pathak, Jalaj},
  year={2021},
  publisher={Indian Institute of Management Bangalore},
  abstract={By January 2021, the stock of GameStop (GME) was heavily shorted by institutional investors but an unprecedented retail campaign for pushing-up its stock price culminated in a short squeeze by the end of January 2021. Adapting recent innovations in text analysis in finance and on microblogging platforms, we present evidence that both the tone and the volume of discussions on the subreddit r/wallstreetbets had significant predictive associations with the GME return, volatility and put-call ratio.}
}

 @misc{subreddit, title={Subreddit stats}, url={https://subredditstats.com/}} 
 
 @misc{davidson_2018, title={Meet the Bros Behind /r/WallStreetBets, Who Lose Hundreds of Thousands of Dollars in a Day—And Brag About It}, url={https://money.com/wall-street-bets/}, journal={Money}, publisher={Money}, author={Davidson, Jake}, year={2018}, month={Oct}}
 
@TechReport{Semenova21,
  author={Winkler, Julian and Semenova, Valentina},
  title={{Reddit's self-organised bull runs: Social contagion and asset prices}},
  year=2021,
  month=Jan,
  institution={Institute for New Economic Thinking at the Oxford Martin School, University of Oxford},
  type={INET Oxford Working Papers},
  url={https://ideas.repec.org/p/amz/wpaper/2021-04.html},
  number={2021-04},
  abstract={This paper develops an empirical and theoretical case for how 'hype' among retail investors can drive large asset fluctuations. We use the dataset of discussions on WallStreetBets (WSB), an online investor forum with over nine million followers as of April 2021, to show how excitement about trading opportunities can ripple through an investor community with large market impacts. This paper finds empirical evidence of psychological contagion among retail investors by exploiting differences in stock price fluctuations and discussion intensity. We show that asset discussions on WSB are self-perpetuating: an initial set of investors attracts a larger and larger group of excited followers. Sentiments about future stock performance also spread from one individual to the next, net of any fundamental price movements. Leveraging these findings, we develop a model for how social contagion impacts prices. The proposed model and simulations show that social contagion has a destabilizing effect on markets. Finally, we establish a causal relationship between WSB activity and financial markets using an instrumental variable approach.},
  keywords={},
  doi={},
}

@article{Schou22,
author = {Schou, Peter Kalum and Bucher, Eliane and Waldkirch, Matthias and Gr\"{u}nwald, Eduard},
title = {We Did Start the Fire: r/wallstreetbets, ‘Flash movements’ and the Gamestop Short-Squeeze},
journal = {Academy of Management Proceedings},
volume = {2022},
number = {1},
pages = {14028},
year = {2022},
doi = {10.5465/AMBPP.2022.32},

URL = { 
        https://doi.org/10.5465/AMBPP.2022.32
    
},
eprint = { 
        https://doi.org/10.5465/AMBPP.2022.32
    
}
,
    abstract = { In January 2021, Wall Street suddenly faced a challenge from an online community, r/wallstreetbets, which organized a large group of small investors in betting against Wall Street hedge funds. In an instant, the online community took on a social movement nature that brought them comparisons to Occupy Wall Street. While scholars are gaining a growing insight into the life of social movements in online communities, current theory does not explain how a movement can suddenly arise in online communities, leaving us with little knowledge to explain how such action - which had critical social impact - arises. To fill this gap, we studied the Wallstreetbets movement relying on a mixed-methods research design, combining an unsupervised topic model with in-depth qualitative coding. Based on this method, we conceptualize Wallstreetbets as a ‘flash movement’, a movement that arises swiftly without former planning or design, through the imbrication of social activities with affordances and constraints of online communities. Our study contributes to (1) the recent interest in spontaneous action in social movements; (2) how social media affordances and constraints affect social movements, and (3) methodologies for studying digital social movements. }
}

%WSB and market returns

@techreport{witts2021irrational,
  title={The Irrational Market: Considering the effect of the online community Wall Street Bets on Financial Market Variables},
  author={Witts, David William and Tortosa-Ausina, Emili and Arribas, Iv{\'a}n and others},
  year={2021},
  abstract={The rise of the Internet, social media and the unfettered access to financial markets has fostered a new era of retail investing. Investing is no longer the activity of the professional, but is available to all, and being exploited to the greatest extent by users of Wall Street Bets. This research considered the implications of retail investors within the Wall Street Bets community on financial markets. Utilising VAR, ARDL and VECM models, we find that Wall Street Bets sentiment provides some incremental investment information, illustrating short-term predictive power over returns of specific assets, and may be beneficial in forecasting short-term volatility and trading volume.}
}

@inproceedings{baumgartner2020pushshift,
  title={The pushshift reddit dataset},
  author={Baumgartner, Jason and Zannettou, Savvas and Keegan, Brian and Squire, Megan and Blackburn, Jeremy},
  booktitle={Proceedings of the international AAAI conference on web and social media},
  volume={14},
  pages={830--839},
  year={2020}
}

@article{chacon2022will,
  title={Will the reddit rebellion take you to the moon? Evidence from WallStreetBets},
  author={Chacon, Ryan G and Morillon, Thibaut G and Wang, Ruixiang},
  journal={Financial Markets and Portfolio Management},
  pages={1--25},
  year={2022},
  publisher={Springer},
  abstract={In early 2021, several stocks receiving attention from retail traders known as “meme stocks” soared in value. A primary source of information regarding these stocks is from the social media platform Reddit, specifically from a subreddit known as WallStreetBets (WSB).This paper investigates whether a simple and easily implementable trading strategy following the WallStreetBets (WSB) subreddit can produce alpha. We document no evidence this is the case. Though we do observe a positive relation between WSB submissions and abnormal trading volume, we find that a portfolio that goes long buy recommendations and short sell recommendations each day is not profitable on a risk-adjusted basis. Holding periods from one day to one year fail to produce alpha. These findings are robust to a variety of different portfolio formation strategies. Our results provide an early look at the data following the explosion of interest in social media inspired retail investing.}
}


@article{Hutto_Gilbert_2014, title={VADER: A Parsimonious Rule-Based Model for Sentiment Analysis of Social Media Text}, volume={8}, url={https://ojs.aaai.org/index.php/ICWSM/article/view/14550}, abstractNote={ &lt;p&gt; The inherent nature of social media content poses serious challenges to practical applications of sentiment analysis. We present VADER, a simple rule-based model for general sentiment analysis, and compare its effectiveness to eleven typical state-of-practice benchmarks including LIWC, ANEW, the General Inquirer, SentiWordNet, and machine learning oriented techniques relying on Naive Bayes, Maximum Entropy, and Support Vector Machine (SVM) algorithms. Using a combination of qualitative and quantitative methods, we first construct and empirically validate a gold-standard list of lexical features (along with their associated sentiment intensity measures) which are specifically attuned to sentiment in microblog-like contexts. We then combine these lexical features with consideration for five general rules that embody grammatical and syntactical conventions for expressing and emphasizing sentiment intensity. Interestingly, using our parsimonious rule-based model to assess the sentiment of tweets, we find that VADER outperforms individual human raters (F1 Classification Accuracy = 0.96 and 0.84, respectively), and generalizes more favorably across contexts than any of our benchmarks. &lt;/p&gt; }, number={1}, journal={Proceedings of the International AAAI Conference on Web and Social Media}, author={Hutto, C. and Gilbert, Eric}, year={2014}, month={May}, pages={216-225} }

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{capm,
Author = {Fama, Eugene F. and French, Kenneth R.},
Title = {The Capital Asset Pricing Model: Theory and Evidence},
Journal = {Journal of Economic Perspectives},
Volume = {18},
Number = {3},
Year = {2004},
Month = {September},
Pages = {25-46},
DOI = {10.1257/0895330042162430},
URL = {https://www.aeaweb.org/articles?id=10.1257/0895330042162430}}

@article{granger,
 ISSN = {00129682, 14680262},
 URL = {http://www.jstor.org/stable/1912791},
 abstract = {There occurs on some occasions a difficulty in deciding the direction of causality between two related variables and also whether or not feedback is occurring. Testable definitions of causality and feedback are proposed and illustrated by use of simple two-variable models. The important problem of apparent instantaneous causality is discussed and it is suggested that the problem often arises due to slowness in recording information or because a sufficiently wide class of possible causal variables has not been used. It can be shown that the cross spectrum between two variables can be decomposed into two parts, each relating to a single causal arm of a feedback situation. Measures of causal lag and causal strength can then be constructed. A generalisation of this result with the partial cross spectrum is suggested.},
 author = {C. W. J. Granger},
 journal = {Econometrica},
 number = {3},
 pages = {424--438},
 publisher = {[Wiley, Econometric Society]},
 title = {Investigating Causal Relations by Econometric Models and Cross-spectral Methods},
 urldate = {2022-09-12},
 volume = {37},
 year = {1969}
}

% twitter fake news
@inproceedings{rosenfeld2020kernel,
  title={A kernel of truth: Determining rumor veracity on twitter by diffusion pattern alone},
  author={Rosenfeld, Nir and Szanto, Aron and Parkes, David C},
  booktitle={Proceedings of The Web Conference 2020},
  pages={1018--1028},
  year={2020}
}

@article{Monti2019,
   author = {Monti, Federico and Frasca, Fabrizio and Eynard, Davide and Mannion, Damon and Bronstein, Michael M},
   title = {Fake news detection on social media using geometric deep learning},
   journal = {arXiv preprint arXiv:1902.06673},
   year = {2019},
   type = {Journal Article}
}


@article{Vosoughi2018,
   author = {Vosoughi, Soroush and Roy, Deb and Aral, Sinan},
   title = {The Spread of True and False News Online},
   journal = {Science (New York, NY)},
   volume = {359},
   number = {6380},
   pages = {1146-1151},
   ISSN = {1095-9203},
   year = {2018},
   type = {Journal Article}
}

% cascade stuff

@article{jasser,
   author = {Jasser, Jasser and Garibay, Ivan and Scheinert, Steve and Mantzaris, Alexander V.},
   title = {Controversial information spreads faster and further than non-controversial information in Reddit},
   journal = {Journal of Computational Social Science},
   volume = {5},
   number = {1},
   pages = {111-122},
   abstract = {Online users discuss and converse about all sorts of topics on social networks. Facebook, Twitter, Reddit are among many other networks where users can have this freedom of information sharing. The abundance of information shared over these networks makes them an attractive area for investigating all aspects of human behavior on information dissemination. Among the many interesting behaviors, controversiality within social cascades is of high interest to us. It is known that controversiality is bound to happen within online discussions. The online social network platform Reddit has the feature to tag comments as controversial if the users have mixed opinions about that comment. The difference between this study and previous attempts at understanding controversiality on social networks is that we do not investigate topics that are known to be controversial. On the contrary, we examine typical cascades with comments that the readers deemed to be controversial concerning the matter discussed. This work asks whether controversially initiated information cascades have distinctive characteristics than those not controversial in Reddit. We used data collected from Reddit consisting of around 17 million posts and their corresponding comments related to cybersecurity issues to answer these emerging questions. From the comparative analyses conducted, controversial content travels faster and further from its origin. Understanding this phenomenon would shed light on how users or organization might use it to their help in controlling and spreading a specific beneficiary message.},
   ISSN = {2432-2725},
   DOI = {10.1007/s42001-021-00121-z},
   url = {https://doi.org/10.1007/s42001-021-00121-z},
   year = {2022},
   type = {Journal Article}
}

% GNNs and similar
@article{GAT,
   author = {Veličković, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Lio, Pietro and Bengio, Yoshua},
   title = {Graph attention networks},
   journal = {arXiv preprint arXiv:1710.10903},
   year = {2017},
   type = {Journal Article}
}

@article{GCN,
   author = {Kipf, Thomas N and Welling, Max},
   title = {Semi-supervised classification with graph convolutional networks},
   journal = {arXiv preprint arXiv:1609.02907},
   year = {2016},
   type = {Journal Article}
}

@article{shervashidze2011weisfeiler,
  title={Weisfeiler-lehman graph kernels.},
  author={Shervashidze, Nino and Schweitzer, Pascal and Van Leeuwen, Erik Jan and Mehlhorn, Kurt and Borgwardt, Karsten M},
  journal={Journal of Machine Learning Research},
  volume={12},
  number={9},
  year={2011}
}

@article{van2008visualizing,
  title={Visualizing data using t-SNE.},
  author={Van der Maaten, Laurens and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={11},
  year={2008}
}

@article{hamilton,
author = {Hamilton, William L.},
title = {Graph Representation Learning},
journal = {Synthesis Lectures on Artificial Intelligence and Machine Learning},
volume = {14},
number = {3},
pages = {1-159},
year = {2020},
doi = {10.2200/S01045ED1V01Y202009AIM046},

URL = { 
        https://doi.org/10.2200/S01045ED1V01Y202009AIM046
    
},
eprint = { 
        https://doi.org/10.2200/S01045ED1V01Y202009AIM046
    
}

}

@article{CascadeAnalysis,
author = {Zhou, Fan and Xu, Xovee and Trajcevski, Goce and Zhang, Kunpeng},
title = {A Survey of Information Cascade Analysis: Models, Predictions, and Recent Advances},
year = {2021},
issue_date = {March 2022},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {54},
number = {2},
issn = {0360-0300},
url = {https://doi.org/10.1145/3433000},
doi = {10.1145/3433000},
abstract = {The deluge of digital information in our daily life—from user-generated content, such as microblogs and scientific papers, to online business, such as viral marketing and advertising—offers unprecedented opportunities to explore and exploit the trajectories and structures of the evolution of information cascades. Abundant research efforts, both academic and industrial, have aimed to reach a better understanding of the mechanisms driving the spread of information and quantifying the outcome of information diffusion. This article presents a comprehensive review and categorization of information popularity prediction methods, from feature engineering and stochastic processes, through graph representation, to deep learning-based approaches. Specifically, we first formally define different types of information cascades and summarize the perspectives of existing studies. We then present a taxonomy that categorizes existing works into the aforementioned three main groups as well as the main subclasses in each group, and we systematically review cutting-edge research work. Finally, we summarize the pros and cons of existing research efforts and outline the open challenges and opportunities in this field.},
journal = {ACM Comput. Surv.},
month = {mar},
articleno = {27},
numpages = {36},
keywords = {information cascade, information diffusion, Popularity prediction}
}

@article{horawalavithana2020cascade,
  title={Cascade-LSTM: Predicting information cascades using deep neural networks},
  author={Horawalavithana, Sameera and Skvoretz, John and Iamnitchi, Adriana},
  journal={arXiv preprint arXiv:2004.12373},
  year={2020}
}

@article{attention,
   author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, Lukasz and Polosukhin, Illia},
   title = {Attention is all you need},
   journal = {arXiv preprint arXiv:1706.03762},
   year = {2017},
   type = {Journal Article}
}
@article{Nyman2018NewsAN,
  title={News and Narratives in Financial Systems: Exploiting Big Data for Systemic Risk Assessment},
  author={Rickard Nyman and Sujit Kapadia and David Tuckett and David Gregory and Paul Ormerod and Robert Smith},
  journal={ERN: Systemic Risk (Topic)},
  year={2018}
}
@article{pivskorec2014cohesiveness,
  title={Cohesiveness in financial news and its relation to market volatility},
  author={Pi{\v{s}}korec, Matija and Antulov-Fantulin, Nino and Novak, Petra Kralj and Mozeti{\v{c}}, Igor and Gr{\v{c}}ar, Miha and Vodenska, Irena and {\v{S}}muc, Tomislav},
  journal={Scientific reports},
  volume={4},
  number={1},
  pages={1--8},
  year={2014},
  publisher={Springer}
}
@misc{grootendorst2022bertopic,
      title={BERTopic: Neural topic modeling with a class-based TF-IDF procedure}, 
      author={Maarten Grootendorst},
      year={2022},
      eprint={2203.05794},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

